A Simple yet Effective Network based on Vision Transformer for Camouflaged Object and Salient Object Detection

Camouflaged object detection (COD) and salient object detection (SOD) are two distinct yet closely-related computer vision tasks widely studied during the past decades. Though sharing the same purpose of segmenting an image into binary foreground and background regions, their distinction lies in the fact that COD focuses on concealed objects hidden in the image, while SOD concentrates on the most prominent objects in the image. Previous works achieved good performance by stacking various hand-designed modules and multi-scale features. However, these carefully-designed complex networks often performed well on one task but not on another. In this work, we propose a simple yet effective network (SENet) based on vision Transformer (ViT), by employing a simple design of an asymmetric ViT-based encoder-decoder structure, we yield competitive results on both tasks, exhibiting greater versatility than meticulously crafted ones. Furthermore, to enhance the Transformer's ability to model local information, which is important for pixel-level binary segmentation tasks, we propose a local information capture module (LICM). We also propose a dynamic weighted loss (DW loss) based on Binary Cross-Entropy (BCE) and Intersection over Union (IoU) loss, which guides the network to pay more attention to those smaller and more difficult-to-find target objects according to their size. Moreover, we explore the issue of joint training of SOD and COD, and propose a preliminary solution to the conflict in joint training, further improving the performance of SOD. Extensive experiments on multiple benchmark datasets demonstrate the effectiveness of our method. The code is available at https://github.com/linuxsino/SENet.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> table/LICM.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of LICM and Convpass \cite{convpass}. “Base” indicates SENet without LICM. “Base + LICM” is essentially SENet. “Base + Convpass” indictes replacing LICM with Convpass. Note that the structure of Convpass does not allow us to perform image reconstruction at the same time, so for a fair comparison, the masking ratios of all three experiments here are set to $0$.}
\resizebox{\linewidth}{!}{\begin{tabular}{cccccccccccccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Settings}} 
& \multicolumn{4}{c|}{COD10K-Test}                     
& \multicolumn{4}{c|}{NC4K}                    
& \multicolumn{4}{c|}{DUTS-Test}                  
& \multicolumn{4}{c}{HKU-IS}      \\ \cline{2-17} 
\multicolumn{1}{c|}{}              
&$S_{\alpha}\uparrow$ &$E_{\phi}\uparrow$  &$F_{\beta}^{\omega}\uparrow$  &\multicolumn{1}{c|}{$M \downarrow$}       
&$S_{\alpha}\uparrow$ &$E_{\phi}\uparrow$  &$F_{\beta}^{\omega}\uparrow$  &\multicolumn{1}{c|}{$M \downarrow$}     
&$S_{\alpha}\uparrow$ &$E_{\phi}\uparrow$  &$F_{\beta}^{m}\uparrow$  &\multicolumn{1}{c|}{$M \downarrow$}   
&$S_{\alpha}\uparrow$ &$E_{\phi}\uparrow$  &$F_{\beta}^{m}\uparrow$    & $M \downarrow$     \\ \hline

\multicolumn{1}{l|}{Base}               
&.860  &.920  &.771  & \multicolumn{1}{c|}{.026} 
&.885  &.930  &.841  & \multicolumn{1}{c|}{.034} 
&.922  &.950  &.920  & \multicolumn{1}{c|}{.024} 
&.941  &.969  &.948  &.021  \\

\multicolumn{1}{l|}{Base + Convpass}               
&.860  &.922  &.770  & \multicolumn{1}{c|}{.026} 
&.888  &.929  &.840  & \multicolumn{1}{c|}{.035} 
&.927  &.949  &.921  & \multicolumn{1}{c|}{.024} 
&.938  &.970  &.950  &.020  \\

\multicolumn{1}{l|}{Base + LICM}               
&.863  &.924  &.780  & \multicolumn{1}{c|}{.025} 
&.887  &.931  &.843  & \multicolumn{1}{c|}{.033} 
&.925  &.951  &.926  & \multicolumn{1}{c|}{.022} 
&.940  &.969  &.953  &.019  \\
 \hline
 
\end{tabular}}
\label{table:licm}
\end{table*}
